Reliable Inference in Edge-Cloud Model Cascades via Conformal Alignment

Edge intelligence enables low-latency inference via compact on-device models, but assuring reliability remains challenging. We study edge-cloud cascades that must preserve conditional coverage: whenever the edge returns a prediction set, it should contain the true label with a user-specified probability, as if produced by the cloud model. We formalize conditional coverage with respect to the cloud predictive distribution, and introduce a conformal alignment-based (CAb) cascading mechanism that certifies this property with user control over the risk level. Our method casts escalation from edge to cloud models as a multiple-hypothesis testing (MHT) problem, tailoring conformal alignment (CA) to select which inputs can be safely handled at the edge. The proposed CAb model cascading method yields statistical guarantees on the average fraction of edge decisions that satisfy cloud-level conditional coverage. The procedure applies to arbitrary edge prediction sets, including variants of conformal prediction (CP), and exposes a tunable trade-off among coverage, deferral rate, and set size. Experiments on CIFAR-100 image classification and the TeleQnA question-answering (QA) benchmark show that the proposed CAb cascade maintains the target conditional coverage for edge predictions while substantially reducing offloading to the cloud and incurring modest increases in prediction-set size.

==> problem_definition_section.tex <==
\section{Problem Definition} \label{sec:problem_definition}

\subsection{Setting}
Consider the edge-cloud system shown in Fig.~1, in which the cloud implements a reference predictive model $p^*(y|x)$, while the edge has access to a low-quality model $p^e(y|x)$, where $x \in \mathcal{X}$ is an input and $y \in \mathcal{Y}$ is a discrete output. The edge-cloud system is tasked to implement a predictive mapping from any input $x$ to a subset $\Gamma(x)$ of the label space $\mathcal{Y}$. The goal is to ensure that the prediction set $\Gamma(x)$ contains the ground-truth label $y$ with probability no smaller than a predetermined coverage level $1-\alpha \in  [0,1]$.

Formally, the target \emph{$(1-\alpha)$-conditional coverage guarantee} for all inputs $x$ processed at the edge-cloud system can be formulated as the inequality 
\begin{align} \label{eq:ideal_goal}
    \Pr[y \in \Gamma(x)|x] \geq 1-\alpha,
\end{align}
where $\Pr[\cdot|x]$ represents the conditional distribution of label $y$ given input $x$. We adopt the cloud predictive distribution $p^*(y|x)$ as the reference distribution of the label $y$ given input $x$, and thus we evaluate the probability in (\ref{eq:ideal_goal}) as
\begin{align} \label{eq:idea_goal_reformula}
    \Pr[y \in \Gamma(x)|x] = p^*(\Gamma(x)|x) = \sum_{y \in \Gamma(x)} p^*(y|x).
\end{align}
Accordingly, the $(1-\alpha)$-conditional coverage guarantee (\ref{eq:ideal_goal}) is achievable by deferring the input $x$ to the cloud. In fact, using the cloud model $p^*(y|x)$, the $(1-\alpha)$-highest density cloud prediction set 
\begin{align} \label{eq:cloud_prediction_set}
    \Gamma^*(x) = \arg \min_{\Gamma^*(x) \subseteq \mathcal{Y}} |\Gamma^*(x)| \text{  s.t. } p^*(\Gamma^*(x)|x) \geq 1-\alpha,
\end{align}
satisfies the condition (\ref{eq:ideal_goal}). The main challenge addressed in this paper is hence how to approximate the conditional coverage condition (\ref{eq:ideal_goal}) while processing as many inputs $x$ as possible at the edge.

\subsection{Design Criteria}
As explained, our goal is to approximate condition (\ref{eq:ideal_goal}) while allowing for some decisions to be carried out at the edge. In the considered edge-cloud system, the prediction set $\Gamma(x)$ is thus given by 
\begin{align} \label{eq:original_prediction}
       \Gamma(x) =
        \begin{cases}
       \Gamma^*(x), & \text{if input $x$ is deferred to the cloud }  \\
       \Gamma^e(x) , & \text{if input $x$ is processed at the edge} ,
        \end{cases}
\end{align}
where $\Gamma^e(x)$ is \emph{any} stochastic prediction set constructed using the edge predictive distribution $p^e(y|x)$, e.g., via conformal prediction \cite{angelopoulos2021gentle}. In general, it is not possible to guarantee the conditional coverage condition (\ref{eq:ideal_goal}) when the prediction set $\Gamma(x)$ differs from the cloud prediction set $\Gamma^*(x)$, unless one chooses the trivial prediction set $\Gamma(x)=\mathcal{Y}$ (see \cite[Sec. 5]{vovk2012conditional} for details). Therefore, we address probabilistic versions of the guarantee (\ref{eq:ideal_goal}) applied to a batch $\mathcal{D}^\text{te}=\{x_i\}_{i=1}^{|\mathcal{D}^\text{te}|}$ of unlabeled test inputs. We specifically consider two versions of condition (\ref{eq:ideal_goal}), with the first providing a closer, but more restrictive approximation and the latter offering a more practical alternative.


\subsubsection{Probabilistic conditional coverage guarantee} The first approximate function for the conditional requirement (\ref{eq:ideal_goal}) imposes that the probability that all of the test inputs $x_i \in \mathcal{D}^\text{te}$ meet the condition (\ref{eq:ideal_goal}) simultaneously is no smaller than a user-defined validity level $1-\delta \in [0,1]$, i.e., 
\begin{align} \label{eq:prob_goal}
    \Pr\big \{ \Pr[y_i \in \Gamma(x_i)|x_i] \geq 1-\alpha, \text{ for all $x_i \in \mathcal{D}^\text{te}$}  \big \} \geq 1-\delta.
\end{align}
In (\ref{eq:prob_goal}), the inner probability is evaluated with respect to the same reference conditional distribution $p^*(y_i|x_i)$ as in (\ref{eq:ideal_goal}), while the outer probability is over the covariates $\{x_i\}_{i=1}^{|\mathcal{D}^\text{te}|}$ of the test input dataset $\mathcal{D}^\text{te}$ and over any reference data used to produce the prediction set $\Gamma(x)$ (see Sec.~IV for details). {\color{red}We can do this FWER controls, since the experiment is similar to FDR controls. But maybe we can remove FWER, since this control is too conservative, meaning deferring almost all of the inputs to the cloud, which is not very meaningful.}

\subsubsection{Average satisfaction rate guarantee} The condition (\ref{eq:prob_goal}), requiring all test inputs to meet the condition (\ref{eq:ideal_goal}), may be practically too strict, resulting in an excessive use of cloud resources. Therefore, we also consider a more relaxed requirement imposing a constraint on the average fraction of test input in $\mathcal{D}^\text{te}$ that satisfy the constraint (\ref{eq:ideal_goal}). This requirement is expressed as 
\begin{align} \label{eq:batch_goal}
\mathbb{E}\bigg[\frac{ | \{x_i \in \mathcal{D}^\text{te}: \Pr[y_i \in \Gamma(x_i)|x_i] \geq 1-\alpha \} | }{|\mathcal{D}^\text{te}|}\bigg] \geq 1-\delta,
\end{align}
where the inner probability is taken with respect to the reference distribution of the label $y_i \sim p^*(y_i|x_i)$ given test input $x_i$, while the outer expectation is evaluated with respect to the covariates $\{x_i\}_{i=1}^{|\mathcal{D}^\text{te}|}$ of the test input dataset $\mathcal{D}^\text{te}$ and over any reference data used to produce the prediction set $\Gamma(x)$. Note that condition (\ref{eq:batch_goal}) coincides with (\ref{eq:prob_goal}) when we have a single test input, i.e., $|\mathcal{D}^\text{te}| =1$.


Since the requirement (\ref{eq:prob_goal}) and (\ref{eq:batch_goal}) can be always met by a selection procedure that defers all inputs to the cloud or that returns the trivial prediction set $\Gamma(x) = \mathcal{Y}$, it is important to evaluate the performance of a cascading scheme in terms of the deferral ratio and of the informativeness of the prediction set.

Denote as $\mathcal{S} \subseteq \mathcal{D}^\text{te}$ the function of test examples processed at the edge. The \emph{deferral ratio} evaluates the expected fraction of the test samples deferred to the cloud, i.e.,
\begin{align} \label{eq:deferral_ratio}
   \text{DR} = \mathbb{E}\left[ 1 - \frac{|\mathcal{S}|}{|\mathcal{D}^{\text{te}}|} \right],
\end{align}
where the expectation is taken with respect to the distribution of the selected subset $\mathcal{S}$ and over any reference data used to generate the prediction set $\Gamma(x)$. The deferral ratio ranges from $0$, indicating that all test samples are processed at the edge, to $1$, indicating that defers all test inputs to the cloud.

The informativeness of the prediction set is evaluated by comparing the set size $|\Gamma(x)|$ with the cloud model's set size $|\Gamma^*(x)|$. Accordingly, the expected size of the prediction set $\Gamma(x)$ normalized by the size of the cloud prediction set, referred to \emph{inefficiency}, is defined as
\begin{align} \label{eq:inefficiency}
     \text{Inef} = \frac{1}{|\mathcal{D}^{\text{te}}|} \mathbb{E}\left[ \sum_{x_i \in \mathcal{D}^{\text{te}}} \frac{|\Gamma(x_i)|}{|\Gamma^*(x_i)|}  \right],
\end{align}
where the expectation is taken over the randomness of the covariates $\{x_i\}_{i=1}^{|\mathcal{D}^\text{te}|}$ of the test input dataset $\mathcal{D}^\text{te}$ and over any reference data used to generate the prediction set $\Gamma(x)$. The inefficiency measures the extent to which the edge-cloud system needs to pay in terms of the prediction set size at the cost of incorporating the cost-efficient edge model. The inefficiency generally ranges from $1$, indicating an edge-cloud system prediction is efficient as the cloud prediction, to $|\mathcal{Y}|$, representing the worst case in which the edge-cloud system returns always the trivial prediction set $\Gamma(x) = \mathcal{Y}$ even in the absence of aleatoric uncertainty, i.e., $|\Gamma^*(x)|=1$ for all test inputs $x$.

% In practice, if the edge model performance is extremely poor, the cascading system can perform no better than deferring all test inputs to the cloud. Therefore, it is also useful to assess the power of the system to discover inputs for which the corresponding edge prediction set $\Gamma^e(x)$ can truly offer reliable decisions, i.e., satisfying the input conditional requirement (\ref{eq:ideal_goal}), defined as 
% \begin{align} \label{eq:power}
%     \text{Power} =  \mathbb{E}\bigg[ \frac{| \{x_i \in \mathcal{S}: p^*(\Gamma^e(x_i)|x_i) \geq 1-\alpha      \}|}{ \max \left( | \{x_i \in \mathcal{D}^\text{te}:  p^*(\Gamma^e(x_i)|x_i) \geq 1-\alpha       \}|  , 1 \right) }  \bigg],
% \end{align}
% where the expectation is evaluated with respect to the distribution of the subset $\mathcal{S}$ and over any reference data used to generate the prediction set $\Gamma(x)$. Intuitively, power captures how often the system correctly utilizes the edge instead of unnecessarily deferring reliable inputs to the cloud. The power ranges from $0$, indicating the worst case that the system fails to select any of the test inputs satisfying the requirement (\ref{eq:ideal_goal}), to $1$, representing that the system perfectly selects all such inputs without missing any.

In short, a well-designed model cascading mechanism should seek to minimize deferral ratio and inefficiency, while satisfying the required guarantees in (\ref{eq:prob_goal}) or (\ref{eq:batch_goal}).





{\color{blue} In this subsection, we will describe the model cascading procedure that satisfies (\ref{eq:FDR}). We will particularly adopt the \emph{sequential screening} viewpoint where the inputs that are likely to violate the coverage condition (\ref{eq:ideal_goal}) are progressively  \emph{screened out} until the remaining, unscreened, inputs satisfy the average condition (\ref{eq:batch_goal_reformulated}). The main desiderata for such screening procedure are: (\emph{i}) sequential screening should not stop if unscreened inputs would violate the average condition  (\ref{eq:ideal_goal}); while (\emph{ii}) it should stop as soon as possible to ensure low deferral rate (\ref{eq:deferral_ratio}).  And the main challenges comes from the absence of knowledge of $C^*(x)$ for the inputs in $\mathcal{D}^\text{te}$. To this end, reference \cite{gui2024conformal} assumed the availability of held-out validation dataset $\{ (x^\text{val}_i, C^*(x^\text{val}_i)) \}_{i=1}^{|\mathcal{D}^{\text{val}}|}$ whose inputs will be augmented with the test inputs $\mathcal{D}^\text{te}$, to provide a guideline for the corresponding screening procedure on when to stop its process. The key idea is to sequentially estimate the FDP of the unscreened \emph{test} inputs based on the available, unscreened, \emph{validation} data; stop whenever such estimate lies below the target level $\delta$. The details of such sequential screening comes next. 


\subsubsection{Sequential Screening}
To elaborate, let us denote as $\mathcal{D}^\text{val}=\{x^\text{val}_i\}_{i=1}^{|\mathcal{D}^\text{val}|}$ the validation inputs. Suppose now that we have some arbitrary screening ordering across the augmented inputs $\mathcal{D}^\text{val}\cup \mathcal{D}^\text{te}$ possibly dependent on such input data, and denote the corresponding ordered $|\mathcal{D}^\text{val}|+|\mathcal{D}^\text{te}|$ number of inputs as
\begin{align} \label{eq:ordering}
    x_{(1)}, x_{(2)}, ..., x_{(|\mathcal{D}^\text{val}+|\mathcal{D}^\text{te}|)}. 
\end{align}
We will detail the choice of such ordering shortly. Accordingly, at each screening step $\ell$, the screened inputs and unscreened inputs can be written as
\begin{align} \label{eq:unscreend_test_inputs}
     \mathcal{D}^{\text{scr}}_{(\ell)} = \{x_{(i)}\}_{i=1}^{\ell}, \quad \quad \mathcal{D}^{\text{uns}}_{(\ell)} = \{x_{(i)}\}_{i=\ell + 1}^{|\mathcal{D}^{\text{val}}|+|\mathcal{D}^{\text{te}}|},
\end{align}
respectively, and the corresponding unscreened validation and test inputs can be expressed as
\begin{align} \label{eq:selected_set}
    \mathcal{D}^{\text{uns,val}}_{(\ell)}  =\mathcal{D}^{\text{uns}}_{(\ell)} \cap \mathcal{D}^{\text{val}}, \quad \quad
    \mathcal{D}^{\text{uns,te}}_{(\ell)}  =\mathcal{D}^{\text{uns}}_{(\ell)} \cap \mathcal{D}^{\text{te}}. 
\end{align}

As mentioned before, the FDP for the test, unscreened, inputs, $\mathcal{D}_{(l)}^\text{uns,te}$ will be estimated using the validataion, unscreened, inputs, $\mathcal{D}_{(l)}^\text{uns,val}$ as follows
\begin{align} \label{eq:FDP_estimator}
    \widehat{\text{FDP}}_{( \ell)} = \frac{|\mathcal{D}^{\text{te}}|}{1 + |\mathcal{D}^{\text{val}}|} \frac{1+| \{x_i \in \mathcal{D}^{\text{uns,val}}_{( \ell)}: C^*(x_i) < 1-\alpha      \}|}{| \mathcal{D}^{\text{uns,te}}_{(\ell)}|},
\end{align}
where the multiplicative term $\frac{|\mathcal{D}^{\text{te}}|}{1 + |\mathcal{D}^{\text{val}}|}$ is to compensate for the discrepancy between the size of calibration and test inputs among the unscreened ones.  

Equipped with the FDP estimate at hand at each screening step $l$, the sequential screening procedure stops whenever the unscreened test inputs are deemed to satisfy the FDP constraint $\delta$, i.e., 
\begin{align} \label{eq:stopping_rule}
    \ell_{\text{CA}} = \inf \{ \ell \geq 0:  \widehat{\text{FDP}}_{( \ell)} \leq \delta \}.
\end{align}
\subsubsection{Theoretical Guarantees}
The unscreened test inputs, i.e., $\mathcal{D}_{(l_\text{CA})}^\text{uns,val}$ will satisfy the FDR constraint (\ref{eq:FDR}) for which we formally state next. 

\textbf{Proposition 1:} \textit{If the examples in the validation dataset $\mathcal{D}^{\text{val}}$, and the test dataset $\mathcal{D}^{\text{te}}$ are exchangeable, e.g., i.i.d., then for any pre-determined tolerated violation rate $\delta \in [0,1]$, the output subset of CA, i.e., edge-processed subset $\mathcal{S} = \mathcal{D}^{\text{uns,te}}_{(\ell_{\text{CA}})}$, can satisfy the average violation rate requirement 
\begin{align} \label{eq:Proposition_1}
     \mathbb{E}\left[\frac{\left| \{ x_i \in \mathcal{S} : C^*(x_i) < 1 - \alpha \} \right|}{|\mathcal{S}|} \right] \leq \delta.
\end{align}
}

The proof of this proposition follows directly from the FDR control of CA (see \cite[Thm.~1]{gui2025acs} for details).



\subsubsection{Choice of Ordering}
We now present the screening ordering (\ref{eq:ordering}) that we consider in this work. To this end, we introduce the alignment score predictor $\hat{C}(x)$ which can be obtained based on some available training dataset $\mathcal{D}^{\text{tr}}= \{ (x^\text{tr}_i, C^*(x^\text{tr}_i)) \}_{i=1}^{|\mathcal{D}^{\text{tr}}|}$.  We can then impose the ordering (\ref{eq:ordering}) based on the predicted alignment scores in an ascending order, i.e., 
\begin{align} \label{eq:screen_order}
    \hat{C}(x_{(1)}) \leq \cdots \leq \hat{C}(x_{(|\mathcal{D}^{\text{val}}|)}) \leq \cdots \leq \hat{C}(x_{(|\mathcal{D}^{\text{val}}|+|\mathcal{D}^{\text{te}}|)}).
\end{align}
Such approach in fact allows one to recover original conformal selection [] built upon the conformal p-values rather than the above described screening procedure, whose choice \emph{per se} is also sensible by noting that inputs that are screened out will never be included in the selected set hence it is desirable to screen out the inputs with lowest predicted alignment scores.
}
